Towards Neural Mixture Recommender for Long Range Dependent User Sequences

Understanding temporal dynamics has proved to be highly valuable for accurate recommendation. Sequential recommenders have been successful in modeling the dynamics of users and items over time. However, while different model architectures excel at capturing various temporal ranges or dynamics, distinct application contexts require adapting to diverse behaviors. In this paper we examine how to build a model that can make use of different temporal ranges and dynamics depending on the request context. We begin with the analysis of an anonymized Youtube dataset comprising millions of user sequences. We quantify the degree of long-range dependence in these sequences and demonstrate that both short-term and long-term dependent behavioral patterns co-exist. We then propose a neural Multi-temporal-range Mixture Model (M3) as a tailored solution to deal with both short-term and long-term dependencies. Our approach employs a mixture of models, each with a different temporal range. These models are combined by a learned gating mechanism capable of exerting different model combinations given different contextual information. In empirical evaluations on a public dataset and our own anonymized YouTube dataset, M3 consistently outperforms state-of-the-art sequential recommendation methods.

==> abstract/abstract.tex <==
\begin{abstract}
On platforms providing a large and diverse catalog of items, the recommendation experience is key for users to be able to discover which items are available that suit their needs and tastes.
Providing accurate recommendations based on sequences of previously observed user/item interactions is therefore a crucial task which is challenged by the length of such sequences and the fact that user behavior is generally influenced by a long term memory. 
In the present paper, we highlight the challenge of capturing latent interests underlying long sequences of user generated data thanks to a production dataset comprising of millions of sequences up to 300 element long and adopt a novel approach to address it.
As a first contribution, we provide a precise quantification of the degree of long range dependence in user generated sequences and demonstrate that both very short term dependent and very long term dependent behavioral patterns co-exist. We then propose a neural Multi-temporal-range Mixture Model~(\emph{M3}) as a tailored solution.
Our novel approach employs a mixture of models -- each with a different temporal range -- whose outputs are combined by a learned gating mechanism capable of using different combinations of models to provide recommendations for our home page as well as item specific pages (in an end-to-end manner). In empirical evaluations on a public dataset and our own production dataset our new model \emph{M3} consistently outperforms state-of-the-art sequential recommendation methods.
\end{abstract}
